Who Are the `Silent Spreaders'?: Contact Tracing in Spatio-Temporal Memory Models

The COVID-19 epidemic has swept the world for over a year. However, a large number of infectious asymptomatic COVID-19 cases (\textit{ACC}s) are still making the breaking up of the transmission chains very difficult. Efforts by epidemiological researchers in many countries have thrown light on the clinical features of ACCs, but there is still a lack of practical approaches to detect ACCs so as to help contain the pandemic. To address the issue of ACCs, this paper presents a neural network model called Spatio-Temporal Episodic Memory for COVID-19 (\textit{STEM-COVID}) to identify ACCs from contact tracing data. Based on the fusion Adaptive Resonance Theory (\textit{ART}), the model encodes a collective spatio-temporal episodic memory of individuals and incorporates an effective mechanism of parallel searches for ACCs. Specifically, the episodic traces of the identified positive cases are used to map out the episodic traces of suspected ACCs using a weighted evidence pooling method. To evaluate the efficacy of STEM-COVID, a realistic agent based simulation model for COVID-19 spreading is implemented based on the recent epidemiological findings on ACCs. The experiments based on rigorous simulation scenarios, manifesting the current situation of COVID-19 spread, show that the STEM-COVID model with weighted evidence pooling has a higher level of accuracy and efficiency for identifying ACCs when compared with several baselines. Moreover, the model displays strong robustness against noisy data and different ACC proportions, which partially reflects the effect of breakthrough infections after vaccination on the virus transmission.

==> LaTeX - ArXiv/alg_acp_detection.tex <==
\begin{algorithm}[!t]
	\caption{Evidence pooling and ACC search.}
	\label{alg:acp_detection}
	
	\KwIn{episodic memory learned in STEM-COVID}
	\KwIn{a threshold of activation value $\delta_c$}
	\KwOut{a set of identified individuals}

	\tcp{\small{Step 1: Evidence activity pooling}}
	reset $F_3$ layer\\\label{alg:acp:merge_start}
	set contribution parameters: $\gamma^e \leftarrow 0, \gamma^c \leftarrow 1$\\\label{alg:acp:gamma_merge}
	present a positivity vector in $F_2$: $\mathbf{c} \leftarrow (1)$\\
	activate $F_3$ using choice function\\\label{alg:acp:activate_positive}
	reset episode field in $F_2$\\
	initialize evidence vector $\mathbf{E} \leftarrow \mathbf{0}$\\\label{alg:acp:unifying_vector_start}
	\ForEach{code $0< T_j \leq 1$ in $F_3$}
	{
		readout node $j$ to episode field: $\mathbf{x}^{e} \leftarrow \mathbf{w}^e_j$\\
		update the evidence vector: $\mathbf{E} \leftarrow \mathbf{x}^{e} \vee \mathbf{E}$\\
		\label{alg:acp:merge_end}
	}
	
	\tcp{\small{Step 2: ACC Search}}
	set contribution parameters: $\gamma^e \leftarrow 1, \gamma^c \leftarrow 1$\\ \label{alg:acp:similarities_start}
	set a positivity vector: $\mathbf{c} \leftarrow (0)$\\\label{alg:acp:set_untested}
	present $\mathbf{E}$ and $\mathbf{c}$ in $F_2$\\\label{alg:acp:activate_unstested_start}
	activate $F_3$ using choice function\\\label{alg:acp:activate_unstested_end}
%	sort the individuals in a descending order of activation values\\
	return IDs of identified individuals $\{j|T_j>\delta_c\}$\\\label{alg:acp:similarities_end}
\end{algorithm}

==> LaTeX - ArXiv/alg_baseline.tex <==
\begin{algorithm}
	\caption{A baseline of computing trace similarities.}
	\label{alg:baseline}
	
	\KwIn{merged events $\{\varepsilon_{t}\}$ of $N_{t}$ $t$-SCCs}
	\KwIn{episodes of $N_{u}$ untested individuals}
	\KwOut{similarity of each untested individual}
	
	\ForEach{untested individual $a_{i=0,1,..., N_{u}-1}$}
	{
		intialize a counter $c \leftarrow 0$\\
		retrieve the episode $e_i=<\varepsilon_0, \varepsilon_1,..., \varepsilon_{T-1}>$\\
		\ForEach{$\varepsilon_j$ in $e_i$}
		{\label{alg:baseline:count_start}
			\ForEach{$\varepsilon_l \in \{\varepsilon_{t}\}$}
			{
				\If{$\varepsilon_j == \varepsilon_l$}
				{
					$c \leftarrow c+1$\\
					break\\
				}
			}
			\label{alg:baseline:count_end}
		}
		calculate the trace similarity $s_i \leftarrow c/T$\\\label{alg:baseline:similarity}
	}

\end{algorithm}

==> LaTeX - ArXiv/alg_episodic_learning.tex <==
\begin{algorithm}[!t]
	\caption{Incremental construction of collective spatio-temporal episodic memory.}
	\label{alg:episodic_learning}
	
	\KwIn{episodes of all $N$ individuals $\{e_i|0 \leq i < N\}$}
	\KwIn{positivity of all individuals: $\{CP_i\}$}
	\KwOut{learned episodic memory in STEM-COVID}
%	\vspace{0.5em}
	
	\ForEach{$e_i = <\varepsilon_0, \varepsilon_1, ..., \varepsilon_{T'}>$}
	{\label{alg:episodic:individual_start}	
		initialize a set of activated codes $Js \leftarrow \varnothing$\\
		
		\tcp{\small{learning in bottom network}}
		\ForEach{$\varepsilon_l = (t_l,p_l)$}
		{\label{alg:episodic:episode_start}
			initialize a code flag: $J \leftarrow -1$\\
			normalize: $t'\leftarrow t_l/T, p' \leftarrow p_l/P$\\\label{alg:episodic:normalize}
			present $\mathbf{I}=((t'), (p'))$ to $F_1$\\\label{alg:episodic:presentF1}
			\ForEach{code $J'$ in episode field in $F_2$}
			{\label{alg:episodic:resonance_event_start}
				\If{a top-down matching between $J'$ and $\mathbf{I}$ succeeds}
				{
					$J \leftarrow J'$\\
					break\\
				}
				\label{alg:episodic:resonance_event_end}
			}
			\If{$J == -1$}
			{
				create a new code $J$ for this new pattern\\\label{alg:episodic:new_event_node}
				expand the field as an input to $F_3$\\
			}
			$Js \leftarrow Js \cup \{J\}$\\
			\label{alg:episodic:episode_end}
		}
		\tcp{\small{learning in top network}}
		form a binary vector $\mathbf{E}$: $\mathbf{E}_j=1$, if $j \in Js$\\\label{alg:episodic:top_start}
		form a positivity vector: $\mathbf{c} = (CP_i)$\\
%		\If{ $i \in C$}
%		{
%			form a positivity vector: $\mathbf{c} \leftarrow (1)$\\
%		}
%		\Else
%		{
%			form a positivity vector: $\mathbf{c} \leftarrow (0)$\\
%		}
		present the input vectors $(\mathbf{E}, \mathbf{c})$ in $F_2$\\
		recruit an uncomitted code $J$ in $F_3$\\
		do an overwrite learning: $\mathbf{w}_J^e=\mathbf{E}$ and $\mathbf{w}_J^c=\mathbf{c}$\\
		\label{alg:episodic:top_end}\label{alg:episodic:individual_end}
	}
\end{algorithm}

==> LaTeX - ArXiv/tab_scenarios.tex <==
\begin{table}[!bt]
	%\renewcommand{\arraystretch}{1.2}
	%\small
	\centering
	%\resizebox{50em}{4.5em}{
	\setlength{\tabcolsep}{1mm}{
		\begin{tabular}{c||c|c|c|c|c|c}
			\toprule
			
			scenarios & $N$ & $P_{vh}$ & $P_h$ & $P_m$ & $P_l$ & $N_{u\_0}$\\
			\midrule

			S200N  & 	200 &	50 &	2 &	10 &	2 &	1(N)\\
			
			S200H  & 	200	&	50 & 	2 & 10 &	2 & 1(H)\\
			
			S1000N &   1000 &  250 &   10 & 50 &   10 & 5(N)\\
			
			\bottomrule
			
	\end{tabular} }
	\vspace{-0.5em}
	\caption{
		Summary of settings in the three scenarios.}
	\label{tab:scen}
\end{table}

==> LaTeX - ArXiv/tab_success_rates_scen1_3.tex <==
\begin{table*}[!bt]
	%\renewcommand{\arraystretch}{1.2}
	%\small
	\centering
	%\resizebox{50em}{4.5em}{
		\begin{tabular}{c||cc|cc|cc}
			\toprule
			
			\multirow{2}{*}{measures} & \multicolumn{2}{c|}{\textbf{ACPs}} & \multicolumn{2}{c|}{\textbf{$c$-ACPs}} & 
			\multicolumn{2}{c}{\textbf{index cases}}\\ 
			
			& scen1 & scen3 & scen1 & scen3  & scen1 & scen3 \\
			\midrule

			top-1 & 30.0\% 	& \textbf{40.0\%}	& 30.0\%	& \textbf{40.0\%}	& \textbf{13.3\%}	& 6.7\%\\
			
			top-3 & \textbf{63.3\%}	& 60.0\% 	& 56.7\%	& \textbf{60.0\%} 	& \textbf{23.3\%}	& 6.7\%\\
			
			top-5 & 70.0\%	& \textbf{80.0\%} 	& 63.3\% 	& \textbf{80.0\%}	& \textbf{26.7\%}	& 20.0\%\\
			
			top-15 & 86.7\%	& \textbf{93.3\%}	& 76.7\%	& \textbf{93.3\%}	& \textbf{43.3\%}	& 33.3\%\\
			
			top-25 & 90.0\%	& \textbf{100.0\%}	& 90.0\%	& \textbf{100.0\%}	& 50.0\%	& \textbf{53.3\%}\\
			
			\bottomrule
			
	\end{tabular} %}
	\caption{
		The identification success rates in the first and third scenarios.}
	\label{tab:success_scen1_3}
\end{table*}

==> LaTeX - ArXiv/tab_time_cost.tex <==
\begin{table}[!bt]
	%\renewcommand{\arraystretch}{1.2}
	%\small
	\centering
	%\resizebox{50em}{4.5em}{
	\setlength{\tabcolsep}{1mm}{
		\begin{tabular}{c||cc|cc|cc}
			\toprule
			
			\multirow{2}{*}{time (s)} & \multicolumn{2}{c|}{\textbf{S200N}} & \multicolumn{2}{c|}{\textbf{S200H}} & 
			\multicolumn{2}{c}{\textbf{S1000N}}\\ 
			
			& ours & baseline & ours & baseline  & ours & baseline \\
			\midrule

			Min 	& 3.1 	& 7.3	& 3.1	& 11.3	& 76.8	& 100.0\\
			
			Mean	& 3.3	& 18.5 & 3.2	& 24.7	& 81.3	& 565.8\\
			
			Max 	& 4.4	& 29.4	& 3.4	& 33.1	& 94.0	& 784.8\\
			
			\bottomrule
			
	\end{tabular} }
	\vspace{-0.5em}
	\caption{
		Time costs for computing trace similarities.}
	\label{tab:time}
\end{table}

==> tab_success_rates_scen1_3.tex <==
\begin{table*}[!bt]
	%\renewcommand{\arraystretch}{1.2}
	%\small
	\centering
	%\resizebox{50em}{4.5em}{
		\begin{tabular}{c||cc|cc|cc}
			\toprule
			
			\multirow{2}{*}{measures} & \multicolumn{2}{c|}{\textbf{ACPs}} & \multicolumn{2}{c|}{\textbf{$c$-ACPs}} & 
			\multicolumn{2}{c}{\textbf{index cases}}\\ 
			
			& scen1 & scen3 & scen1 & scen3  & scen1 & scen3 \\
			\midrule

			top-1 & 30.0\% 	& \textbf{40.0\%}	& 30.0\%	& \textbf{40.0\%}	& \textbf{13.3\%}	& 6.7\%\\
			
			top-3 & \textbf{63.3\%}	& 60.0\% 	& 56.7\%	& \textbf{60.0\%} 	& \textbf{23.3\%}	& 6.7\%\\
			
			top-5 & 70.0\%	& \textbf{80.0\%} 	& 63.3\% 	& \textbf{80.0\%}	& \textbf{26.7\%}	& 20.0\%\\
			
			top-15 & 86.7\%	& \textbf{93.3\%}	& 76.7\%	& \textbf{93.3\%}	& \textbf{43.3\%}	& 33.3\%\\
			
			top-25 & 90.0\%	& \textbf{100.0\%}	& 90.0\%	& \textbf{100.0\%}	& 50.0\%	& \textbf{53.3\%}\\
			
			\bottomrule
			
	\end{tabular} %}
	\caption{
		The identification success rates in the first and third scenarios.}
	\label{tab:success_scen1_3}
\end{table*}
